TypedSchematics: A Block-based PCB Design Tool with Real-time Detection of Common Connection Errors

Within PCB design, the reuse of circuit design blocks is a major preventing factor inhibiting beginners from reusing designs made by experts, a common practice in software but non-existent in circuit design at large. Despite efforts to improve reusability (e.g. block-based PCB design) by platforms such as SparkFun ALC and Altium Upverter, they lack merging techniques that safely guide users in connecting different circuit blocks without requiring assistance from third-party engineers. In this paper, we propose TypedSchematics, a block-based standalone PCB design tool that supports beginners create their own PCBs by providing a language syntax for typing circuit blocks with circuit data that addresses multiple challenges, from real-time detection of connection errors to automated composition and user-scalable libraries of circuit blocks. Through a user study, we demonstrate TypedSchematics improvements in design support for merging circuit blocks compared to Fusion 360. Three PCBs designed with TypedSchematics further showcase our tool capabilities, one designed by high school students demonstrates the potential of TypedSchematics to significantly lower the PCB design skill-floor.

==> background.tex <==
%auto-ignore
\section{Background}
\label{sec:background}



==> impl.tex <==
%auto-ignore
\section{System}
\label{sec:system}
% (Implementation) and following the relaxed JSON format (cite relaxed).
